High-performance sampling of generic Determinantal Point Processes

Determinantal Point Processes (DPPs) were introduced by Macchi as a model for repulsive (fermionic) particle distributions. But their recent popularization is largely due to their usefulness for encouraging diversity in the final stage of a recommender system. The standard sampling scheme for finite DPPs is a spectral decomposition followed by an equivalent of a randomly diagonally-pivoted Cholesky factorization of an orthogonal projection, which is only applicable to Hermitian kernels and has an expensive setup cost. Researchers have begun to connect DPP sampling to $LDL^H$ factorizations as a means of avoiding the initial spectral decomposition, but existing approaches have only outperformed the spectral decomposition approach in special circumstances, where the number of kept modes is a small percentage of the ground set size. This article proves that trivial modifications of $LU$ and $LDL^H$ factorizations yield efficient direct sampling schemes for non-Hermitian and Hermitian DPP kernels, respectively. Further, it is experimentally shown that even dynamically-scheduled, shared-memory parallelizations of high-performance dense and sparse-direct factorizations can be trivially modified to yield DPP sampling schemes with essentially identical performance. The software developed as part of this research, Catamari, https://hodgestar.com/catamari, is released under the Mozilla Public License v2.0. It contains header-only, C++14 plus OpenMP 4.0 implementations of dense and sparse-direct, Hermitian and non-Hermitian DPP samplers.

==> figures/aztec_40.tex <==
\begin{figure}

\begin{subfigure}{0.5\textwidth}
\centering
\includegraphics[width=2.4in]{images/aztec-40-0-d.png}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\centering
\includegraphics[width=2.4in]{images/aztec-40-1-d.png}
\end{subfigure}

\caption{Two samples from the Aztec diamond DPP of order 40, defined via a
complex, non-Hermitian kernel based upon Kenyon's formula over the Kasteleyn
matrix. Their likelihoods are both $\text{exp}(-568.381)$.}

\end{figure}


==> figures/aztec_5.tex <==
\begin{figure}

\begin{subfigure}{0.5\textwidth}
\centering
\includegraphics[width=2.4in]{images/aztec-5-0-d.png}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\centering
\includegraphics[width=2.4in]{images/aztec-5-1-d.png}
\end{subfigure}

\caption{Two samples from the Aztec diamond DPP of order 5, defined via a
complex, non-Hermitian kernel based upon Kenyon's formula over the Kasteleyn
matrix. Their likelihoods are both $\text{exp}(-10.3972)$.}

\end{figure}


==> figures/aztec_5_0.tex <==
\begin{figure}

\caption{A sample from the Aztec diamond DPP, defined via a complex,
non-Hermitian kernel based upon Kenyon's formula over the Kasteleyn matrix.
Its sample likelihood is $\text{exp}(-10.3972)$.}

\centering
\includegraphics[width=2.7in]{images/aztec-5-0-d.png}

\end{figure}


==> figures/aztec_5_1.tex <==
\begin{figure}

\caption{A sample from the Aztec diamond DPP, defined via a complex,
non-Hermitian kernel based upon Kenyon's formula over the Kasteleyn matrix.
Its sample likelihood is $\text{exp}(-10.3972)$.}

\centering
\includegraphics[width=2.7in]{images/aztec-5-1-d.png}

\end{figure}


==> figures/laplacian_2d_0_75.tex <==
\begin{figure}
\begin{subfigure}{0.5\textwidth}
\includegraphics[width=2in]{images/shifted_laplacian-200-0_75-0.png}
% 0.0124 seconds.
\caption{Sample with log-likelihood of $-27612.6$.}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\includegraphics[width=2in]{images/shifted_laplacian-200-0_75-ml-0.png}
% 0.0114 seconds.
\caption{MAP sample with log-likelihood of $-26009$.}
\end{subfigure}
\end{figure}

